When is Memorization of Irrelevant Training Data Necessary for High-Accuracy Learning?

Modern machine learning models are complex and frequently encode surprising amounts of information about individual inputs. In extreme cases, complex models appear to memorize entire input examples, including seemingly irrelevant information (social security numbers from text, for example). In this paper, we aim to understand whether this sort of memorization is necessary for accurate learning. We describe natural prediction problems in which every sufficiently accurate training algorithm must encode, in the prediction model, essentially all the information about a large subset of its training examples. This remains true even when the examples are high-dimensional and have entropy much higher than the sample size, and even when most of that information is ultimately irrelevant to the task at hand. Further, our results do not depend on the training algorithm or the class of models used for learning. Our problems are simple and fairly natural variants of the next-symbol prediction and the cluster labeling tasks. These tasks can be seen as abstractions of text- and image-related prediction problems. To establish our results, we reduce from a family of one-way communication problems for which we prove new information complexity lower bounds. Additionally, we present synthetic-data experiments demonstrating successful attacks on logistic regression and neural network classifiers.

==> abstract.tex <==

\begin{abstract} 
    Modern machine learning models are complex and frequently encode surprising amounts of information about individual inputs. In extreme cases, complex models appear to memorize entire input examples, including seemingly irrelevant information (social security numbers from text, for example). In this paper, we aim to understand whether this sort of memorization is necessary for accurate learning. We describe natural prediction problems in which every sufficiently accurate training algorithm must encode, in the prediction model,  essentially all the information about a large subset of its training examples. This remains true even when the examples are high-dimensional and have entropy much higher than the sample size,
    and even when most of that information is ultimately irrelevant to the task at hand. Further, our results 
    do not depend on the training algorithm or the class of models used for learning. 
    
    Our problems are simple and fairly natural variants of the next-symbol prediction and the cluster labeling tasks. These tasks can be seen as abstractions of text- and image-related prediction problems. To establish our results, we reduce from a family of one-way communication problems for which we prove new information complexity lower bounds. 
\end{abstract}



==> appendices/minimax.tex <==
\subsection{From Average-Case to Worst-Case via Minimax}\label{sec:minimax}

We provide metadistributions (dependent on the sample size $n$ and dimension $d$) upon which any near-optimal algorithm has high information cost.
A metadistribution is over problem instances, each of which is itself a distribution over labeled examples.
The ``easy'' direction of von Neumann's Minimax Theorem allows us to turn this into a worst-case guarantee. 

\begin{proposition}\label{prop:worst_case}
    Suppose $q^*$ is a metadistribution such that any algorithm that is $\eps$-suboptimal for Learn($n,N,q^*,\pi$) satisfies $I(X;M\mid P)=\Omega(nd)$. Then, for any $\alg$ that is $\eps$-suboptimal, there exists a problem instance $p^*\in \Delta(\mc{X})$ such that
    \begin{align*}
        I(X;M \mid P=p^*) \geq I(X;M|P) = \Omega(nd).
    \end{align*}
\end{proposition}
\begin{proof}
    Since $I(X;M|P)=\E_{p\sim q^*}[I(X;M\mid P=p)]$ is an expectation, there always exists a problem instance whose value is at least that of the expectation.
\end{proof}

The assumption of Propostion~\ref{prop:worst_case} deserves some discussion.
%
Specifically, recall that a learning algorithm $\alg$ is $\eps$-suboptimal for Learn($n,N,q_{n,d},\pi$) if it competes with the best possible learner $\Aopt^{(n,d)}$ for  $q_{n,d}$ when receiving a sample of size $n$. An equivalent requirement is that the error of $\alg$ on $p$ be close that that of $\Aopt^{(n,d)}$ on average over instances $p\sim q_{n,d}$. On one hand,  this assumption is much weaker than assuming that $\alg$ is near-optimal for each instance $p$ (since we compare with the learner $\Aopt^{(n,d)}$ whose average error over $p\sim q_{n,d}$ is lowest, not a learner that is tailored to $p$). On the other hand, it is not obviously comparable to the requirements of properness and consistency made by \citet{bassily2018learners,nachum2018direct}. 
% For one thing, our learning problems are not all defined in terms of PAC learning of a concept class. Some of our learning problems do generate instances that are realizable by a VC-bounded class; however, for those learning problems, the sample size 
For one thing, not all of our learning tasks fit neatly into the framework of PAC learning.
For those that do, the sample size $n$ that we consider is generally less than (or comparable to) the VC-dimension of the underlying concept class---too low to guarantee that every proper and consistent learner has high accuracy. Understanding the full relationship between these different kinds of assumptions is a subject for future work. 





==> appendices/related_work.tex <==
\section{Related Work}
\label{sec:related_work}

\subsection{Main Writing}

\paragraph{Empirical Work on Sample Memorization in Deep Learning.}

\paragraph{Differential Privacy.}

\paragraph{Representation Dimension.}
A line of work closely related to the topics studied here is that of \emph{representation dimension}, which arises in the analysis of the sample complexity of private PAC (and agnostic) learning as defined in \cite{kasiviswanathan2011can}.
For a given concept class $C$, \cite{beimel2010bounds} define an $\epsilon$-representation of $C$ as a class of functions $\mathcal{H}$ which, for every data distribution $D$ and every concept $c\in C$, there is an $h\in\mathcal{H}$ such that $\Pr_{x\sim D}[h(x)\neq c(x)]\le \epsilon$.
Such a representation may be much smaller than the concept class itself (it may be finite even when $C$ is infinite) and can be privately learned with $O(\log |\mathcal{H}|)$ samples.
This notion is generalized in \cite{beimel2019characterizing} to that of a probabilistic representation, where $\mathcal{H}$ is chosen randomly from a set and need only be a representation of $C$ with high probability.
In \cite{beimel2019characterizing} the authors show that this characterizes the sample complexity of pure private learning. 

In \cite{feldman2014sample} the connection between representation and communication is made explicit, since a learning algorithm outputting a hypothesis in $\mathcal{H}$ needs exactly $\log |\mathcal{H}|$ bits to specify which one.
The authors prove the equivalence of the sample complexity of differentially-private learning and the randomized one-way communication complexity of evaluating concepts and prove additional bounds using this equivalence.

In our learning settings the labels may not be a deterministic function of the inputs.
This is a feature of machine learning in practice but places us outside the classical settings of PAC or agnostic learning.
Nevertheless, we can compare the guarantees of private learning with our lower bounds.
Similarly to agnostic learning (and in contrast to the PAC model) the learning algorithms we analyze may output arbitrary messages.
Private PAC learning asks for guarantees for worst-case concepts and distributions.
The lower bounds from representation dimension are of the form: for any private learning algorithm using too few samples, there is a choice of distribution $D$ and concept $c$ such that the algorithm will produce a bad hypothesis with high probability.
We provide a joint meta-distribution over data distributions and (randomized) labeling functions such that any learning algorithm will low mutual information will have high error. 

\paragraph{VC Dimension.}
The Vapnik-Chervonekis (VC) dimension of a concept class $C$ is well-known to characterize the sample complexity of PAC and agnostic learning in the absence of privacy.

\paragraph{Time-Space Tradeoffs for Learning.}
A line of work beginning with Raz \cite{raz2018fast} (see \cite{garg2018extractor} for a more recent summary of results) establishes time-space tradeoffs for learning: problems where any learning algorithm requires either a large memory or a large number of samples.
The prime example is parity learning over $d$ bits, which is shown to require either $\Omega(d^2)$ bits of memory or exponentially many samples.
The straightforward algorithm for parity learning requires $O(d)$ samples, so this result shows that any feasible algorithm must store, up to constant factors, as many bits as are required to store the dataset.

Our work sets a specific number of samples under which learning is feasible and, for that number of samples, establishes an information lower bound on the \emph{output} of the algorithm.
This implies not only a communication lower bound but also one on memory usage: the algorithm must store the output immediately prior to releasing it.
Some of our models exhibit the property that, with additional data, an algorithm can output a substantially smaller model.
These learning tasks might exhibit a time-space tradeoff, although not as dramatic as the requirement of exponentially many samples.
Intuitiviely, the underlying concept in parity learning must be learned ``all at once,'' since for example the learner's belief about the bits in the second half of the string depend heavily on its belief about the bits in the first half.
Our problem instances seem to have the property that they can be learned ``piece-by-piece,'' where the algorithm learns a chunk of bits independently of the rest of the sample.

\paragraph{Tracing Attacks.}

\paragraph{Data Interpolation in Deep Learning.}

\paragraph{Information Bottleneck.}


\subsection{Lists of related work}

\subsection{Prior work on memorization}

\begin{itemize}
    \item Empirical work on memorizing whole samples
    \begin{itemize}
        \item \bibentry{carlini2018secret}
        \item \bibentry{radhakrishnan2019overparameterized}
        \item \bibentry{zhang2019identity}
        \item \bibentry{nagarajan2018theoretical}
    \end{itemize}
    \item Theory and empirical work on interpolation and label fitting 
    \begin{itemize}
        \item \bibentry{feldman2020does}
        \item \bibentry{zhang2016understanding}
        \item \bibentry{liang2019multiple}
        \item Much much more...
        \item Important distinction: ``just'' labels?
    \end{itemize}
    \item Privacy, reconstruction, and tracing
    \begin{itemize}
        \item \bibentry{dinur2003revealing}
        \item "Exposed!" survey of attacks on privacy
        \item Those papers aren't really about leaking of entire data vectors; rather they show how to recover single bits about individuals (either "their data bit" or membership). 
    \end{itemize}
    \item Relevant highlights of learning + information theory
    \begin{itemize}
        \item ``Information bottleneck'' analyzes representation of data points, doesn't directly apply here
        \begin{itemize}
            \item Our work gives a different type of information bottleneck in learning
        \end{itemize}
    \item Raz et al.'s line of work on time-space lower bounds in learning
    \begin{itemize}
        \item Looks at space during learning (as opposed to what's in the final model).
        \item If time permits: connect our results to that setting?
    \end{itemize}
    \item Work on representation dimension {\color{red} think more about what to say here}
        \begin{itemize}
            \item Beimel, Brenner, Kasiviswanathan, Nissim '1x, Beimel-Nissim-Stemmer '13,  Feldman-Xiao 
                        \begin{itemize}
                            \item (Part of nice line of work on private learning)
                        \end{itemize}
            \item Major points:            
            \begin{itemize}
                \item Representation dimension captures space/info complexity of the worst-case distribution (for a given concept class)
                \item If concept class and example distribution are fixed, space bounded by size of a distribution-specific cover. 
            \end{itemize}
            \item Interesting consequence: for intervals and LTF's,  learning from minimal number of sample (=VC dimension) can require a hypothesis of size $\Omega(n H(X))$, where $H(X)$ can be arbitrarily large.
        \end{itemize}
    
        \end{itemize}

\end{itemize}

\subsection{Work used or cited in our technical results}

\begin{itemize}
    \item String Completion
    \begin{itemize}
        \item \bibentry{bar2004sketching}
        \item \bibentry{feldman2014sample}
    \end{itemize}
    \item Gap Hamming
    \begin{itemize}
        \item \bibentry{indyk2003tight}
        \item \bibentry{hadar2019communication}
        \item \bibentry{ankitsemail}
        \item Braverman paper stating problem is open (cited in email to Mark)
        \item \bibentry{ahlswede1976spreading}
    \end{itemize}
    \item OR of Equalities
    \begin{itemize}
        \item \bibentry{saglam2013communication}
    \end{itemize}
    \item General reference
    \begin{itemize}
        \item \bibentry{mitzenmacher2017probability} 
        \item \bibentry{cover1991elements}
        \item \bibentry{roughgarden2015communication}
        \item \bibentry{guruswami2012essential}
    \end{itemize}
\end{itemize}

\subsection{Other Background}

\begin{itemize}
    \item \bibentry{dagan2016trading}
    \item \bibentry{fei2006one}
    \item \bibentry{lake2011one}
\end{itemize}

==> sections/OREQ.tex <==
\section{Large Alphabet Cluster Identification}\label{sec:OREQ}

Our final task also asks the learning algorithm to identify the cluster from which the test sample arose.

\subsection{Task Description and Error Upper Bound}

Samples consists of length-$d$ strings over alphabets of size $t$, which we will assume without loss of generality to be the integers $[t]$.
Each subpopulation $j$ is defined by an index $i_j\in [d]$ and symbol $\sigma_j\in [t]$.
Every sample from subpopulation $j$ will contain $\sigma_j$ at location $i_j$, and the other entries will be chosen independently and uniformly from $[t]$.
We will take $t = ckd$, for some constant $c$.
Note that there is no explicit noise, but the irrelevant features are filled in randomly.

Two strings from subpopulation $j$ will always match at position $i_j$ and, if the alphabet is sufficiently large, will match nowhere else with high probability.
With multiple samples from a single subpopulation, the learner can reliably infer $i_j$ and $\sigma_j$, encoding just this information in the model.
With just a single sample, though, the learner has no information about the key index, and can only hope to determine it after seeing the test instance.


\begin{rem}
    The above algorithm sends $d\log t$ bits per singleton example it receives.
    We will later show this is, at least asymptotically, required for low error.
    Note that the problem instance, per subpopulation, is defined by the pair $(i_j,\sigma_j)$,
    Note that, given 2 samples from a single subpopulation $j$, with probability at most $\frac{d}{t}=\frac{1}{ck}$, the index/symbol pair $(i_j, \sigma_j)$ can be learned exactly, since all other indices will disagree across the two samples.
    Sending $(i_j, \sigma_j)$ requires only 
\end{rem}

\subsection{Data has Large Entropy}

\subsection{Lower Bound for Singletons-Only}

For any $k$, let ProductTask($k$) be: Alice gets $k$ i.i.d. samples from $[t]^d$, Bob gets one uniform sample.
The label is a promise problem: ProductTask$(X,y)=j$ only if Bob's sample matches exactly one $X_j$ of Alice's in exactly one location.
Otherwise anything Bob outputs is correct.
We want $t=\Theta(dk)$ so this happens with constant probability.
\begin{conj}
    For any $k$, any algorithm $\alg$ solving ProductTask($k$) that satisfies
    \begin{align*}
        \Pr[\text{$\alg$ errs}] \le \epsilon_k
    \end{align*}
    also satifies
    \begin{align*}
        I(X; M)&\ge k d \log t \cdot g(\epsilon_k),
    \end{align*}
    for some convex and nonincreasing $g(\epsilon)$.
\end{conj}

\begin{lemma}
    Suppose for all (or sufficiently small?) $\eps$ there exists a set $B_{\eps_k}\subseteq [t]^d\times[t]^d$ such that
    \begin{align}
        \Pr_y[\mathrm{ProductTask}(X,y)\neq\mathrm{ProductTask}(X',y)\mid (X,X')\notin B_{\eps_k}] \ge \alpha.
    \end{align}
    Then we have that any algorithm $\alg$ solving ProductTask($k$) that satisfies
    \begin{align*}
        \Pr[\text{$\alg$ errs}] \le \epsilon_k
    \end{align*}
    also satifies
    \begin{align*}
        I(X; M)&\ge k d \log t \left(1 - \frac{\log |B_{\eps_k}|}{2kd\log t}\right)\left(1 - \frac{2\epsilon_k}{\alpha}\right).
    \end{align*}
    If we can set $\alpha \ge \sqrt{\epsilon_k}$ this becomes
    \begin{align*}
        I(X; M)&\ge k d \log t \left(1 - \frac{\log |B_{\eps_k}|}{2kd\log t}\right)\left(1 - 2\sqrt{\eps_k}\right),
    \end{align*}
    which is closer to being convex in $\eps_k$.
\end{lemma}

Regard $(x,x')$ as a table with $2k$ rows and $d$ columns, filled with symbols from $t$.
Test sample $Z$ will interact with each column independently.
\begin{itemize}
    \item $B$ will be the set of bad tables (bad for us, the thm provers). We want $|B|$ small.
    \item $G$ will be the set of good tables, with $\delta \cdot d$ good columns. We want $|G|$ big.
    \item A good column has $\gamma\cdot k$ entries distinct {\bf in each half-table}, both $x$ and $x'$.
    \item Pick good column $i\in [d]$. $\Pr[Z \text{ matches } i] \ge \frac{\gamma 2k}{t}$.
    \item If there are $\delta d$ good columns,
        \begin{align}
            \Pr_Z[Z \text{ matches two } i\neq j] \ge \binom{\delta d}{2} \left(\frac{\gamma 2k }{t}\right)^2 \ge (\delta \gamma)^2 (dk/t)^2.
        \end{align}
    \item $dk/t$ will be a constant, so could set $\delta = \gamma = (\eps_k)^{1/4}$ for the $\sqrt{\eps_k}$ behavior we want.
\end{itemize}

Show there are few $B$ bad tables.
\begin{itemize}
    \item Probability that a column is bad? Tossing $2k$ balls into $t$ bins, $2k(1-\gamma)$ bad tosses.
    \begin{align}
        p = \Pr[\text{col bad}]  &\le \binom{2k}{(1-\gamma)2k\gamma} \left(\frac{2k}{t}\right)^{(1-\gamma)2k}
    \end{align}
    \item Prob that table is bad, $\ge \delta d$ bad cols
    \begin{align}
        \Pr[\text{table bad}] &\le \binom{d}{\delta d} p^{\delta d} \\
            &\le \binom{d}{\delta d} \binom{2k}{(1-\gamma)2k\gamma}^{\delta d} \left(\frac{2k}{t}\right)^{(1-\gamma)2\delta kd}.
    \end{align}
\end{itemize}


\subsection{old}

% In our next learning task the samples consists of length-$d$ strings over alphabets of size $t$, which we will assume without loss of generality to be the integers $[t]$.
% Each sample is drawn i.i.d. from a mixture over $k$ subpopulations, where subpopulation $j$ is defined by an index $i_j\in [d]$ and symbol $\sigma_j\in [t]$.
% Every sample from subpopulation $j$ will contain $\sigma_j$ at location $i_j$, and the other entries will be chosen independently and uniformly.
% The learner's task is to identify the cluster label.

% Two strings from subpopulation $j$ will always match at position $i_j$ and, if the alphabet is sufficiently large, will match nowhere else with high probability.
% Thus, with multiple samples from a single subpopulation, the learner can reliably infer $i_j$ and $\sigma_j$, encoding just this information in the model.
% With just a single sample, though, the learner has no information about the key index, and can only hope to determine it after seeing the test instance.
% Intuitively, then, the learning algorithm must encode the singleton examples to achieve high accuracy at this task.

% \begin{thm}
%     {\bf Set parameters here.} 
%     Any algorithm that succeeds on this task with probability $1-\epsilon$ has mutual information
%     \begin{align*}
%         \ldots
%     \end{align*}
% \end{thm}

% We prove this via a reduction to a related problem, where Alice gets $k$ independent samples in $[t]^d$, Bob's is also independent, and he must answer which, if any, of Alice's inputs his input is close to.
% This setting is easier to handle: the joint distribution over Alice and Bob's inputs is a product distribution, and the function to compute is deterministic.
% The key insight in this reduction is that, conditioned on Bob's input matching at least one of Alice's inputs, the joint distribution matches a subproblem of the original task.

% Let us name the three problems, all of which take as inputs strings in $[t]^d$.
% \begin{itemize}
%     \item{\bf DatasetInference($n,k$):} Alice gets $n$ samples drawn i.i.d. from a mixture over $k$ clusters.
%         Clusters are defined by a hidden index/symbol pair, with all other indices picked uniformly at random.
%         Bob tries to infer which of the clusters his sample was drawn from.
%     \item{\bf SingletonsInference($k$):} Alice gets $k$ samples, one from each cluster.
%         Bob tries to infer which of the clusters his sample was drawn from.
%     \item{\bf SingletonsFunction($k$):} Alice gets $k$ strings drawn i.i.d. from the uniform distribution over $[t]^d$. 
%         Bob must compute which of Alice's inputs his string \emph{matches}, where matching is defined as having Hamming distance \emph{exactly} $d-1$.
%         This definition of matching excludes pairs which match in multiple locations.
%         We set this up as a promise problem: Bob needs only output the correct index when his sample matches exactly one of Alice's inputs in exactly one location. 
%         If it matches zero or multiple of Alice's inputs he is always correct.
% \end{itemize}

% Naturally, these three problems are closely related, which we formalize in the following two lemmas.
% \begin{lemma}\label{lemma:OREQ_dataset_singleton}
%     For any protocol $\alg$ solving DatasetInference($k,k$) to error $\epsilon_1$, there is a protocol $\alg'$ solving SingletonsInference($k/3$) to error at most $4 \epsilon_1$.
%     Furthermore, the information cost of $\alg$ is greater than that of $\alg'$.
% \end{lemma}
% \begin{lemma}\label{lemma:OREQ_inference_cluster}
%     Assume $t\ge cdk$ for some constant $c$.
%     Any protocol $\alg$ solving SingletonsInference($k'$) to error $\epsilon_2$ also solves, without modification, SingletonsFunction($k'$) to error $c\epsilon_2$.
% \end{lemma}
% \begin{proof}[Proof of Lemma \ref{lemma:OREQ_dataset_singleton}]
%     $\alg'$ will generate $2k/3$ independent cluster centers and samples $2k/3$ ``fake'' data points from them.
%     Combined with the $k/3$ inputs given to $\alg'$, this will result in a dataset of $k$ points from $k$ subpopulations: exactly the input $\alg$ expects.
%     It is identically distributed to the input to DatasetInference($k,k$), since clusters (defined by a hidden index and symbol) are generated i.i.d. and data points from different clusters are independent.
%     Since $\alg$ may not be symmetric with respect to cluster labels, $\alg'$ relabels the data points according to a random permutation.
    
%     The error of $\alg'$ will be exactly the error of $\alg$ conditioned on (1) $\alg$'s input containing at least $k/3$ singletons and (2) the test instance coming from one of the singletons.
%     Let $S$ be the number of singletons, and $E$ the event that the test instance comes from a singleton clsuter.
%     Since $\epsilon_1$ is the overall error of $\alg$, we have 
%     \begin{align*}
%         \epsilon_1 &= \Pr[\text{$\alg$ errs} \mid S\ge k/3\cap E]\Pr[S\ge k/3\cap E] \\
%                     &\quad+ \Pr[\text{$\alg$ errs}\mid S< k/3\cup \bar{E}]\Pr[S< k/3\cup \bar{E}] \\
%             &\ge \epsilon_2 \Pr[E \mid S\ge k/3] \Pr[S\ge k/3].
%     \end{align*}
%     We have $\Pr[E\mid S\ge k/3]\ge \frac{1}{3}$ since the test instance's clusters is chosen uniformly.
%     Using the Poisson approximation and a Chernoff bound, we can show that 
%     \begin{align*}
%         \Pr[S\ge k/3] \ge 1- e\sqrt{k}e^{-\Omega(k)} \ge \frac{3}{4},
%     \end{align*}
%     for sufficiently large $k$.
%     Thus $\Pr[\text{$\alg'$ errs}] = \epsilon_2 \le 4\epsilon_1$.
% \end{proof}
% \begin{proof}[Proof of Lemma \ref{lemma:OREQ_inference_cluster}]
%     Let $G\subseteq [t]^{kd}\times [t]^d$ be the set of ``good'' singletons/test instance pairs $(x,y)$ that satisfy the promise in SingletonsFunction($k$): in exactly one location, $y$ shares a symbol with exactly one of Alice's inputs. 
%     All other indices in $y$ have symbols that are unique in that index.
%     By definition, the error of a protocol for SingletonsFunction($k$) is exactly the error on this set $G$, where the error is computed w.r.t. the uniform distribution over $G$.
%     We will show that, conditioned on the inputs to SingletonsInference($k$) falling in $G$, the distribution over dataset/input pairs is also uniform.
%     Thus for any protocol $\alg$ we have
%     \begin{align*}
%         \Pr[&\text{$\alg$ errs on SingletonsFunction($k$)}\mid (X,Y)\in G] \\ 
%             &= \Pr[\text{$\alg$ errs on SingletonsInference($k$)}\mid (X,Y)\in G],
%     \end{align*}
%     which allows us to write
%     \begin{align*}
%         \Pr[&\text{$\alg$ errs on SingletonsInference($k$)}] \\ &\ge \Pr[\text{$\alg$ errs on SingletonsInference($k$)}\mid (X,Y)\in G] \Pr[(X,Y)\in G].
%     \end{align*}
%     To bound $\Pr[(X,Y)\in G]$ under the mixture model, we need to bound the probability of matches beyond the fixed cluster match.
%     With $d-1$ ``free'' locations in $y$, each of which might match (with probability $\frac{1}{t}$) any of the $k$ singleton data points, we can apply the union bound to get $\Pr[(X,Y)\in G]\le \frac{dk}{t} \le \frac{1}{c}$.
    
%     It remains to show, under the mixture arising from SingletonsInferences($k$), that $\Pr[(X,Y)=(x,y)\mid (X,Y)\in G]$ is uniform over $G$.
%     First note that, by construction, $\Pr[X=x]$ is uniform, so we turn to $\Pr[Y=y\mid X=x]$.
%     Let random variables $I\in [d]$ and $J\in [k]$ be the index of $y$ and the index of the sample that are chosen to match, so that $y(i)=x_j(i)$.
%     For any $(x,y)$ we have
%     \begin{align*}
%         \Pr[Y=y\mid X=x] &= \sum_{i,j} \Pr[I=i]\cdot \Pr[J=j] \cdot \Pr[Y=y\mid X=x,I=i,J=j] \\
%             &= \frac{1}{kd} \sum_{i,j} \Pr[Y=y\mid X=x,I=i,J=j].
%     \end{align*}
%     If $y(i) = x_j(i)$, then $\Pr[Y=y\mid X=x,I=i,J=j]= \frac{1}{t^{d-1}}$.
%     Otherwise the probability is 0, and since by the definition of $G$ there is exactly 1 pair $(i,j)$ such that $y(i)=x_j(i)$, for all $(x,y)\in G$ we have
%     \begin{align*}
%         \Pr[(X,Y)=(x,y)\mid G] &= \Pr[X=x] \cdot \Pr[Y=y\mid X=x, (X,Y)\in G] \\ 
%             &=  \frac{1}{t^{kd}}\cdot \frac{1}{kd\cdot t^{d-1}},
%     \end{align*}
%     which is independent of $(x,y)$ and thus uniform.
% \end{proof}

% Now we provide our lower bound on SingletonsFunction($k$) directly.
% \begin{lemma}
%     For any algorithm $\alg$ solving SingletonsFunction($k$) to error $\epsilon_3$, we have
%     \begin{align*}
%         I(X;M)\ge H(X) \cdot \left(1 - \frac{\log |B_p|}{2 kd \log t}\right) \cdot \left(1 - \frac{2\epsilon_3}{\alpha}\right).
%     \end{align*}
%     We can bound
%     \begin{align*}
%         |B_q| \le t^{2kd} \left(1 - \left(1 - \frac{2 \mathrm{Vol}(p)}{t^d}\right)^{2k}\right),
%     \end{align*}
%     where $\mathrm{Vol}(p)$ is the Hamming ball (in $[t]^d$) of radius $pd$, and
%     \begin{align*}
%         \alpha \ge \frac{2d}{t^2} \left(1 - 2kp\right) e^{-\frac{3k}{t}}.
%     \end{align*}
%     This holds for any $p\in(0,1)$.
% \end{lemma}
% \begin{proof}
%     Consider the following experiment: after receiving Alice's message $m$ and test instance $y$, Bob samples two i.i.d. datasets $x,x'\sim X\mid M=m$ and computes the function $f$ on them.
%     Recall that, in SingletonsFunction($k$), $f(x,y)$ is only defined when $y$ matches exactly one sample in $x$ in exactly one location.
%     Let $E$ and $E'$, respectively, be the events that $f(X,Y)$ and $f(X',Y)$ are defined.
%     A Bob will compute and output some answer $j^*$.
%     Since $X$ and $X'$ are both distributed identically to the true dataset, we have
%     \begin{align}
%         \Pr[E,E',f(X,Y)\neq f(X',Y)\mid M=m] &\le \Pr[E,f(X,Y)\neq j^*\mid M=m] \nonumber \\
%             &\quad+ \Pr[E,f(X,Y)\neq j^*\mid M=m] \nonumber \\
%             &= 2\Pr[\text{error}\mid M=m]. \label{eq:OREQ_dist_event_error}
%     \end{align}
%     We will now work to lower bound $\Pr[E,E',f(X,Y)\neq f(X',Y)\mid M=m]$.
%     To do this, we will define a set $B_p\subseteq [t]^d\times [t]^d$ parameterized by some $q\in(0,1)$ that is (a) very small relative to $[t]^d\times [t]^d$ and (b) such that, when $(X,X')\notin B_p$, there is a signficant chance of $E$, $E'$, and $f(X,Y)\neq f(X',Y)$.
%     Thus, to achieve low error, the distribution $(X,X')\mid M=m$ must be concentrated on $B_p$, and therefore have low entropy.
    
%     It will be easier to define the complement $\bar{B_p}$.
%     Let $\bar{B_p}$ be the set of pairs $(x,x')$ such that there exist indices $i\neq j$ such that
%     \begin{itemize}
%         \item[(i)] for all $\ell$, $d(x_i,x_\ell') > (1-p)d$.
%         \item[(ii)] for all $\ell$, $d(x_j',x_\ell) > (1-p)d$.
%         \item[(iii)] for all $\ell\neq i$, $d(x_i,x_\ell) > (1-p)d$.
%         \item[(iv)] for all $\ell\neq j$, $d(x_j',x_\ell') > (1-p)d$.
%     \end{itemize}
%     These conditions mean $x_i$ and $x_j'$ are ``isolated'' from all the other data points in both data sets, sharing at most $pd$ indices.
    
%     Define the ``distinghuishing event'' $D = \{E \cap E' \cap f(X,Y)\neq f(X',Y)\}$.
%     We have 
%     \begin{align}
%         \Pr[D\mid M=m] \ge \Pr[D\mid (X,X')\notin B_p, M=m]\Pr[(X,X')\notin B_p\mid M=m].
%         \label{eq:OREQ_dist_event_broken}
%     \end{align}
%     We will lower bound each of these terms.
%     The first we can lower bound with the probability that $Y$ matches $x_i$ in exactly one location, $x_j'$ in exactly one location, and nothing anywhere else.
%     Both of those have at least $d - (2k-1)pd \ge d(1-2kp)$ ``free'' indices, where there is no overlap with any of the data points.
%     To construct a $y$ that satisfies the conditions, then, we pick a location to match $x_i$, a location to match $x_j'$, and fill in the remaining $d-2$ locations with unused symbols, of which there are at least $t-2k$ for each location.
%     This yields
%     \begin{align*}
%         \Pr[D\mid (X,X')\in \bar{B_p}, M=m] &\ge \frac{2d(1-2kp) \left(t - 2k\right)^{d-2} }{t^d} \\
%             &\ge \frac{2d(1-2kp)}{t^2} \exp\left\{-\frac{2kd}{t}\right\} \triangleq \alpha,
%     \end{align*}
%     defining $\alpha$ for concision.
    
%     Now we will lower-bound $\Pr[(X,X')\in \bar{B_q}]$ using the conditional entropy $H(X\mid m)$.
%     We define indicator random variable $A$ that is 1 when $(X,X')\in \bar{B_q}$ and let $q = \Pr[A=1\mid M=m]= \Pr[(X,X')\in \bar{B_q}\mid M=m].$
%     Since $X\perp X'\mid M$, with a little manipulation we can expand:
%     \begin{align*}
%         2H(X\mid M=m) &= H(X,X'\mid M=m) \\
%             &=H(X,X', A\mid M=m) \\
%             &= H(X,X'\mid A, M=m) + H(A\mid M=m) \\
%             &= q \cdot H(X,X'\mid A=1, M=m) \\
%                 &\quad+ (1-q)\cdot H(X,X'\mid A=0, M=m) \\
%                 &\quad+ H(A\mid M=m) \\
%             &\le q \log t^{2kd} + (1-q) \log |B_q| + 1.
%     \end{align*}
%     Thus we can lower bound
%     \begin{align*}
%         \Pr[(X,X')\in \bar{B_q}] = q \ge \frac{2 H(X\mid M=m) - \log |B_q| - 1}{2kd \log t - \log |B_q|}.
%     \end{align*}
%     Combining these results with Equations \eqref{eq:OREQ_dist_event_error} and  \eqref{eq:OREQ_dist_event_broken}, we get
%     \begin{align*}
%         2 \Pr[\text{error}\mid M=m]\ge \alpha \left(\frac{2 H(X\mid M=m) - \log |B_q| - 1}{2kd \log t - \log |B_q|}\right).
%     \end{align*}
%     Since $\E_m\left[\Pr[\text{error}\mid M=m]\right]=\epsilon$, we can take the expectation over $m$ and rearrange to upper bound the conditional entropy.
%     \begin{align*}
%         2H(X\mid M) \le \frac{2\epsilon}{\alpha}\left(2H(X) - \log |B_q|\right) + \log |B_q| + 1.
%     \end{align*}
%     We can turn this into a cleaner lower bound on the mutual information.
%     \begin{align*}
%         I(M;X) = H(X) - H(X\mid M) &\ge H(X) - \frac{2\epsilon}{\alpha}\left( H(X) - \frac{1}{2}\log |B_p|\right) + \frac{1}{2}\log |B_p| + \frac{1}{2} \\
%             &= H(X) \left(1 -\frac{\log |B_p|}{2H(X)}\right)\left(1-\frac{2\epsilon}{\alpha}\right).
%     \end{align*}
    
%     We now need to upper bound $|B_q| = t^{2kd} - |\bar{B_p}|$.
%     To build a pair in $\bar{B_p}$, we select $x_i$ arbitrarily, then $x_j'$ cannot be in the Hamming ball around $x_i$, and then the other $2(k-1)$ choices cannot be in the Hamming balls near those two.
%     Thus 
%     \begin{align*}
%         |\bar{B_q}| &\ge t^d \cdot \left(t^d - \mathrm{Vol}(p)\right)\cdot \left(t^d - 2\mathrm{Vol}(p)\right)^{2k-2)} \\
%             &\ge t^d \cdot \left(t^d - 2\mathrm{Vol}(p)\right)^{2k-1}
%     \end{align*}
%     and 
%     \begin{align*}
%         |B_q| \le t^{2kd} \left( 1 - \left(1 - \frac{2\mathrm{Vol}(p)}{t^d}\right)^{2k-1} \right).
%     \end{align*}
% \end{proof}



==> sections/selected_proofs.tex <==
% \section{Selected Lower Bounds}\label{sec:selected_proofs}

% In this section, we prove the basic information complexity lower bounds necessary for our results in Next-Symbol Prediction and Hypercube Labeling.

% \section{Single Subpopulation Lower Bound for Next-Symbol Prediction}
\section{Next-Symbol Prediction}\label{sec:STOC_NSP}


We now present the information complexity lower bound for Next-Symbol Prediction.
Recall from Example~\ref{ex:nsp} that each data point comes with a subpopulation identifier.
This fact allows us to focus on the ``one-shot'' communication game, where Alice receives a single example. 
The lower bound for $\mathrm{Singletons}(k,q_{NSP})$ is then exactly $k$ times the lower bound for $\mathrm{Singletons}(1,q_{NSP})$.

The core of this proof is based on an existing lower bound \citep{bar2004information,feldman2014sample} for \textit{Augmented Index}, a well-known communication complexity task.
\begin{lemma}\label{lemma:SC_one_shot}
    Fix a noise level $\delta\in [0,1)$.
    For any $\eps_1< \frac{(1-\delta)^2}{4}$, any learning algorithm $\alg$ that is $\eps_1$-suboptimal on \sing{1}{q_{NSP}}  satisfies
    \begin{align*}
        I(X; M)&\ge \frac{d+1}{2} \left(1 - h\left(\frac{2 \epsilon_1}{(1-\SCnoise)^2}\right)\right).
    \end{align*}
\end{lemma}

% Recall that the length of Alice's input is random variable $L$, which is uniform over $[d]$.
% Alice receives $\frac{d+1}{2}$ bits on average, so as $\eps_1\to 0$ this lower bound approaches $H(X)-H(L)=H(X\mid L)$.
% The $\log d$ gap, then, comes from the fact that Alice need not expose the length of her input.

\input{proofs/nsp_singletons.tex}

% \section{Nearest-Neighbor Lower Bound for Hypercube Labeling}
\section{Hypercube Learning}\label{sec:STOC_GHP}

We turn to the lower bound for $\sing{k}{q_{HC}}$, the communication game associated with Hypercube Labeling.
As discussed above in Example~\ref{ex:nearest_neighbor_revisted}, $\sing{k}{q_{HC}}$ is equivalent to the following communication game, which removes the need to analyze the set of fixed indices.
\begin{definition}[Nearest of $k$ Neighbors]
    Alice receives $k$ strings $x_1,\ldots, x_k \in \bit{d}$, drawn i.i.d.~from the uniform distribution.
    Bob receives a string $y\sim BSC_{\frac{1-\rho}{2}}(x_{j})$ for some index $j\in [k]$, also chosen uniformly at random.
    They succeed if Bob outputs $j$.
    % \hfill $\blacksquare$
    \terminalbox
\end{definition}

\begin{lemma}\label{lemma:HC_communication_bound_body}
    Set $\rho=\frac{c\sqrt{\ln n}}{\sqrt{d}}$ for any $n>1$ and constant $c>\sqrt{2}$.
    For every $k\le n$, any one-way communication protocol for Nearest of $k$ Neighbors with error at most $\eps_k \le \frac{1}{10}$ satisfies
    \begin{align*}
        I(X;M) &\ge \frac{kd}{c^2\ln 2}\cdot \frac{\log k}{\log n} \cdot \left(1 - 2h(\epsilon_k)\right).
    \end{align*}
\end{lemma}

\input{proofs/ghp_singletons.tex}




